Dynamic O(arboricity) coloring in polylogarithmic worst-case time

A recent work by Christiansen, Nowicki, and Rotenberg provides dynamic algorithms for coloring sparse graphs, concretely as a function of the arboricity alpha of the input graph. They give two randomized algorithms: O({alpha} log {alpha}) implicit coloring in poly(log n) worst-case update and query times, and O(min{{alpha} log {alpha}, {alpha} log log log n}) implicit coloring in poly(log n) amortized update and query times (against an oblivious adversary). We improve these results in terms of the number of colors and the time guarantee: First, we present an extremely simple algorithm that computes an O({alpha})-implicit coloring with poly(log n) amortized update and query times. Second, and as the main technical contribution of our work, we show that the time complexity guarantee can be strengthened from amortized to worst-case. That is, we give a dynamic algorithm for implicit O({alpha})-coloring with poly(log n) worst-case update and query times (against an oblivious adversary).

==> macros_camera_ready.tex <==
%\documentclass[11pt]{article}
\iffalse
\usepackage[IL2]{fontenc}

\usepackage{amsmath, amssymb, amsthm, amsfonts}
\usepackage{amscd}
\usepackage{mathrsfs}

\usepackage{comment} % \begin{comment}\end{comment} to comment stuff that may be uncommented later on
%\usepackage[shortlabels]{enumitem} % \begin{enumerate}[(a)] % DONT USE it breaks normal enumerate environments so use \item[(A)] instead
%\usepackage{cite}  % DONT USE it clashes with something else in PODC submissions
\usepackage{ifthen}
% \usepackage{arrayjobx}
\usepackage{tikz}
\usetikzlibrary{positioning,decorations.pathreplacing}
\usepackage{ bbold }
%\usepackage{url}
\usepackage{appendix}
\usepackage{graphicx}
\usepackage{color}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{epstopdf}
\usepackage{wrapfig}
\usepackage{paralist}
\usepackage{wasysym}
%\usepackage{float}
%\usepackage{pgf}
\usepackage[textsize=tiny]{todonotes}
%[textsize=tiny] normally
%[disable] to disable

\usepackage{listings} % listing code
% e.g. \begin{lstlisting}[language=Python] for python

%\setlength{\marginparwidth}{2cm}
%apparently can fix todonotes if they are outside of the page

\newcommand{\mtodo}[1]{\todo[color=blue!20]{#1}}

\usepackage{pdflscape} % \clearpage\begin{landscape}...\end{landscape}\clearpage for landscape page


\usepackage{framed}
\usepackage[framemethod=tikz]{mdframed}
\usepackage[bottom]{footmisc}
\usepackage{enumitem}
\setitemize{noitemsep,topsep=3pt,parsep=3pt,partopsep=3pt}
%\usepackage{multirow}
\usepackage[font=small]{caption}
%\captionsetup{font=small}
\usepackage{xspace}

\usepackage{thmtools} % not sure what is it good for but probably has to do something with thm-restate
\usepackage{thm-restate} % \begin{restatable}{theorem}{thmmain}..\end{restatable}
% and then \thmmain*
% common error: \begin{restatable}{theorem}[thmmain]


% CL: Moved this here so it is ``seen'' by hyperref. Otherwise I got ``destination with same identifier'' issues for all theorems, lemmas, etc. with an up-to-date latex installation at home (worked on the crappy out-of-date one at work, though :D).

\usepackage{hyperref}
\hypersetup{
    unicode=false,          % non-Latin characters in Acrobat’s bookmarks
    colorlinks=true,        % false: boxed links; true: colored links
    linkcolor=red,          % color of internal links (change box color with linkbordercolor)
    citecolor=darkgreen,        % color of links to bibliography
    filecolor=magenta,      % color of file links
    urlcolor=cyan           % color of external links
}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{meta-theorem}[theorem]{Meta-Theorem}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{question}[theorem]{Question}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\fi
\usepackage[capitalize, nameinlink,noabbrev]{cleveref}
%capitalize capitalizes the first letter
%nameinlink probably puts the name in link

%\crefformat{footnote}{#2\footnotemark[#1]#3}
\crefname{theorem}{Theorem}{Theorems}
\crefname{proposition}{Proposition}{Propositions}
\crefname{observation}{Observation}{Observations}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{claim}{Claim}{Claims}
\crefname{problem}{Problem}{Problems}
\crefname{conjecture}{Conjecture}{Conjectures}
\crefname{question}{Question}{Questions}
\crefname{example}{Example}{Examples}
\crefname{fact}{Fact}{Facts}
%--------------------------------------------------------------------

\definecolor{darkgreen}{rgb}{0,0.5,0}

\usepackage{algcompatible}
\algnewcommand\algorithmicswitch{\textbf{switch}}
\algnewcommand\algorithmiccase{\textbf{case}}

% New "environments"
\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{\algorithmicswitch\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicswitch}%
\algdef{SE}[CASE]{Case}{EndCase}[1]{\algorithmiccase\ #1}{\algorithmicend\ \algorithmiccase}%
\algtext*{EndSwitch}%
\algtext*{EndCase}%
%----------------------------------------------------------------------

\newcommand{\fA}{\mathcal{A}}
\newcommand{\fB}{\mathcal{B}}
\newcommand{\fC}{\mathcal{C}}
\newcommand{\fD}{\mathcal{D}}
\newcommand{\fE}{\mathcal{E}}
\newcommand{\fF}{\mathcal{F}}
\newcommand{\fG}{\mathcal{G}}
\newcommand{\fH}{\mathcal{H}}
\newcommand{\fI}{\mathcal{I}}
\newcommand{\fJ}{\mathcal{J}}
\newcommand{\fK}{\mathcal{K}}
\newcommand{\fL}{\mathcal{L}}
\newcommand{\fM}{\mathcal{M}}
\newcommand{\fN}{\mathcal{N}}
\newcommand{\fO}{\mathcal{O}}
\newcommand{\fP}{\mathcal{P}}
\newcommand{\fQ}{\mathcal{Q}}
\newcommand{\fR}{\mathcal{R}}
\newcommand{\fS}{\mathcal{S}}
\newcommand{\fT}{\mathcal{T}}
\newcommand{\fU}{\mathcal{U}}
\newcommand{\fV}{\mathcal{V}}
\newcommand{\fW}{\mathcal{W}}
\newcommand{\fX}{\mathcal{X}}
\newcommand{\fY}{\mathcal{Y}}
\newcommand{\fZ}{\mathcal{Z}}

\newcommand{\tA}{\mathtt{A}}
\newcommand{\tB}{\mathtt{B}}
\newcommand{\tC}{\mathtt{C}}
\newcommand{\tD}{\mathtt{D}}
\newcommand{\tE}{\mathtt{E}}
\newcommand{\tF}{\mathtt{F}}
\newcommand{\tG}{\mathtt{G}}
\newcommand{\tH}{\mathtt{H}}
\newcommand{\tI}{\mathtt{I}}
\newcommand{\tJ}{\mathtt{J}}
\newcommand{\tK}{\mathtt{K}}
\newcommand{\tL}{\mathtt{L}}
\newcommand{\tM}{\mathtt{M}}
\newcommand{\tN}{\mathtt{N}}
\newcommand{\tO}{\mathtt{O}}
\newcommand{\tP}{\mathtt{P}}
\newcommand{\tQ}{\mathtt{Q}}
\newcommand{\tR}{\mathtt{R}}
\newcommand{\tS}{\mathtt{S}}
\newcommand{\tT}{\mathtt{T}}
\newcommand{\tU}{\mathtt{U}}
\newcommand{\tV}{\mathtt{V}}
\newcommand{\tW}{\mathtt{W}}
\newcommand{\tX}{\mathtt{X}}
\newcommand{\tY}{\mathtt{Y}}
\newcommand{\tZ}{\mathtt{Z}}

\newcommand{\ta}{\mathtt{a}}
\newcommand{\tb}{\mathtt{b}}
\newcommand{\tc}{\mathtt{c}}
\newcommand{\td}{\mathtt{d}}
\newcommand{\te}{\mathtt{e}}
\newcommand{\tf}{\mathtt{f}}
\newcommand{\tg}{\mathtt{g}}
\newcommand{\tth}{\mathtt{h}}
\newcommand{\ti}{\mathtt{i}}
\newcommand{\tj}{\mathtt{j}}
\newcommand{\tk}{\mathtt{k}}
\newcommand{\tl}{\mathtt{l}}
\newcommand{\tm}{\mathtt{m}}
\newcommand{\tn}{\mathtt{n}}
\newcommand{\tto}{\mathtt{o}}
\newcommand{\tp}{\mathtt{p}}
\newcommand{\tq}{\mathtt{q}}
\newcommand{\tr}{\mathtt{r}}
\newcommand{\ts}{\mathtt{s}}
\newcommand{\ttt}{\mathtt{t}}
\newcommand{\tu}{\mathtt{u}}
\newcommand{\tv}{\mathtt{v}}
\newcommand{\tw}{\mathtt{w}}
\newcommand{\tx}{\mathtt{x}}
\newcommand{\ty}{\mathtt{y}}
\newcommand{\tz}{\mathtt{z}}

\newcommand{\del}{\textrm{del}}


\newcommand{\JUSTIFY}[1]{\mbox{\fbox{\tiny#1}}\quad}
\newcommand{\eps}{\varepsilon}
\newcommand{\DAS}{$\mathsf{DAS}$\xspace} 
\newcommand{\congestion}{$\mathsf{congestion}$\xspace} 
\newcommand{\dilation}{$\mathsf{dilation}$\xspace} 
\newcommand{\congest}{$\mathsf{CONGEST}\xspace$ }
\newcommand{\local}{$\mathsf{LOCAL}\xspace$ }
\newcommand{\rlocal}{\mathsf{RLOCAL}\xspace}
\newcommand{\rlocaln}{\mathsf{RLOCAL}^{-n}\xspace}
\newcommand{\localn}{\mathsf{LOCAL}^{-n}\xspace}
\newcommand{\tail}{\mathsf{TAIL}\xspace}
\newcommand{\lca}{\mathsf{LCA}\xspace}
\newcommand{\volume}{\mathsf{VOLUME}\xspace}
\newcommand{\ffiid}{\mathsf{FFIID}\xspace}
\newcommand{\tow}{\mathrm{tower}}
\newcommand{\pspace}{\mathsf{PSPACE}}
\newcommand{\ksi}{\xi}
\newcommand{\sgn}{\operatorname{\text{{\rm sgn}}}}
\renewcommand{\P}{\textrm{P}}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\e}{\textrm{e}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\polylg}{\operatorname{polylog}}
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\lglg}{\operatorname{loglog}}
\newcommand{\hopDiameter}[1]{\mathrm{Hop}\-\mathrm{Diam}(#1)}
\newcommand{\shortcutQuality}[1]{\mathrm{Shortcut}\-\mathrm{Quality}(#1)}

\renewcommand{\phi}{\varphi}
\newcommand{\argmin}{\textrm{argmin}}


\newcommand{\E}{\textrm{E}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\Fq}{\mathbb{F}_q}
\newcommand{\prob}[1]{P(#1)}
\newcommand{\Prob}[1]{P\left(#1\right)}
\newcommand{\NumOfLayers}{L}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\Hd}{\operatorname{hd}}
\newcommand{\Wd}{\operatorname{wd}}
\newcommand{\WD}{\operatorname{WD}}
\newcommand{\SPD}{\operatorname{SPD}}
\newcommand{\lev}{\textrm{lev}}
\newcommand{\id}{{\textrm{id}}}


\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}

\renewcommand{\paragraph}[1]{\vspace{0.15cm}\noindent {\bf #1}:}

%--------------------------- Full Or Short --------------------------------------------- ---------------------------------------------------------------------------------------- ----------------------------------------------------------------------------------------

\newcommand{\separate}[1]{\clearpage #1\clearpage} %This is for printing purposes while writing/editing

